On the (Statistical) Detection of Adversarial Examples

Machine Learning (ML) models are applied in a variety of tasks such as network intrusion detection or Malware classification. Yet, these models are vulnerable to a class of malicious inputs known as adversarial examples. These are slightly perturbed inputs that are classified incorrectly by the ML model. The mitigation of these adversarial inputs remains an open problem. As a step towards understanding adversarial examples, we show that they are not drawn from the same distribution than the original data, and can thus be detected using statistical tests. Using thus knowledge, we introduce a complimentary approach to identify specific inputs that are adversarial. Specifically, we augment our ML model with an additional output, in which the model is trained to classify all adversarial inputs. We evaluate our approach on multiple adversarial example crafting methods (including the fast gradient sign and saliency map methods) with several datasets. The statistical test flags sample sets containing adversarial inputs confidently at sample sizes between 10 and 100 data points. Furthermore, our augmented model either detects adversarial examples as outliers with high accuracy (> 80%) or increases the adversary's cost - the perturbation added - by more than 150%. In this way, we show that statistical properties of adversarial examples are essential to their detection.

==> abstract.tex <==
%!TEX root = main.tex

\subsection*{Abstract}
Machine Learning (ML) models are applied in a variety of tasks such as network
intrusion detection or malware classification. Yet, these models are vulnerable
to a class of malicious inputs known as adversarial examples. These are slightly
perturbed inputs that are classified incorrectly by the ML model. The mitigation
of these adversarial inputs remains an open problem.

As a step towards a model-agnostic defense against adversarial examples, we show
that they are not drawn from the same distribution than the original data, and
can thus be detected using statistical tests. As the number of malicious points
included in samples presented to the test diminishes, its detection confidence
decreases. Hence, we introduce a complimentary approach to identify specific
inputs that are adversarial among sets of inputs flagged by the statistical
test. Specifically, we augment our ML model with an additional output, in which
the model is trained to classify all adversarial inputs.

We evaluate our approach\footnote{The code necessary to reproduce our results is
available in the following GitHub repository: \texttt{URL} blinded for
submission.} on multiple adversarial example crafting methods (including the
fast gradient sign and saliency map methods) with several
datasets. The statistical test flags sample sets containing adversarial inputs
confidently at sample sizes between $10$ and $100$ data points. Furthermore, our augmented model either detects
adversarial examples as outliers with high accuracy ($>80$\%) or increases the adversary's
cost---the perturbation added---by more than $150$\%. In this way, we show that
statistical properties of adversarial examples are essential to their detection.

==> macros.tex <==
%!TEX root = main.tex
%%Names
\newcommand{\F}{\ensuremath{f}\xspace}
\newcommand{\A}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\X}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\J}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\Y}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\Z}{\ensuremath{\mathbf{Z}}\xspace}
\newcommand{\T}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\classes}{\ensuremath{\mathbf{\mathcal{Y}}}\xspace}
\newcommand{\samples}{\ensuremath{\mathbf{\mathcal{X}}}\xspace}
%\newcommand{\data}{D\xspace}
%\newcommand{\datas}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\poison}{P\xspace}
\newcommand{\classifiers}{\ensuremath{\mathbf{\mathcal{F}}}\xspace}
%\newcommand{\dist}{\ensuremath{\mathsf{dist}}}
\newcommand{\loss}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\sign}{\ensuremath{\mathsf{sign}}\xspace}
\newcommand{\error}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\threshold}{\textsc{threshold}\xspace}

\newcommand{\out}{\ensuremath{\mathsf{out}}}
\newcommand{\dist}{D\xspace}
\newcommand{\real}{\ensuremath{\mathsf{real}}\xspace}
\newcommand{\train}{\ensuremath{\mathsf{train}}\xspace}

\newcommand{\adv}{\ensuremath{\mathsf{adv}}\xspace}

\newcommand{\monly}{\texttt{manifest\-only}\xspace}
\newcommand{\onlyf}{\texttt{only\-freq}\xspace}
\newcommand{\onlys}{\texttt{only\-small}\xspace}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\DeclareMathOperator*{\argmin}{\mathsf{arg\,min}}
\DeclareMathOperator*{\argmax}{\mathsf{arg\,max}}
\DeclareMathOperator*{\grad}{\mathsf{grad}}
\newcommand{\cm}[1]{\ifdraft\textcolor{red}{\fi \bfseries #1\ifdraft}\fi}

==> taxonomy.tex <==
%!TEX root = main.tex
\label{section:taxonomy}
The adversaries considered in our work span the class of \emph{causative} attacks~\cite{barreno2006can}. The general strategy is two-fold:  (1) the adversary perturbs the training data, and (2) this causes the machine learning classifier to  produce erroneous outputs during its inference phase. This strategy is implementable under many variants, which we thus arrange around three thrusts: adversarial goals, model related capabilities, and training data related capabilities. The resulting taxonomy is adapted to formalize the space of adversaries against machine learning at training time. It complements previous work by Bareno et al.~\cite{barreno2006can}, which studied adversarial machine learning at a more coarse-grained level, and Mei et al.~\cite{Mei:2015:UMT:2886521.2886721}, which proposed the machine teaching framework. A discussion of related work, which complements the elements given below to illustrate our taxonomy, can be found in Section~\ref{section:related-work}.

To understand how a poisoning attack could benefit a party with malicious intentions, consider for instance, actively mislabeling spam email to mislead a spam detection system based on learning or wrongly labeling images submitted to Facebook to mislead Facebook's face recognition system.

One important factor is naturally the actual training algorithm that we want to attack. Depending on whether the underlying optimization problem is linear, convex or non-convex, different attack methodologies can be applied. In this paper, we focus on deep neural networks with non-linear activation functions, which implies a non-convex optimization for training.

\begin{figure}
	\label{fig:poisoning-taxonomy}
	\includegraphics[width=\columnwidth]{poisoning-taxonomy}
	\caption{Taxonomy of Adversaries against Machine Learning at Training Time: attacks are sorted by increasing difficulty along each axis.}
\end{figure}

\boldpara{Adversarial Goals}
Let $\F_D$ be the classifier learned by the training algorithm $\A$ upon complete processing of a training dataset $D$. The adversary manipulates the dataset $D$ in order to cause $\F_D$ to match an expected behavior. Its goal may be to: 
\begin{itemize}
	\item reduce the accuracy of classifier $\F_D$ at test time~\cite{DBLP:conf/icml/BiggioNL12, kloft2010online, perdisci2006misleading}
	\item bring the accuracy down to random performance
	\item change the classifier's output for a specific input:~\cite{nelson2008exploiting}
	\item completely swap classes learned:~\cite{newsome2006paragraph,chung2006allergy,nelson2008exploiting}
\end{itemize}

Having characterized the adversarial goals, we now need to specify which capabilities are needed to achieve them, both in terms of the classifier model and its training dataset. 

\boldpara{Model Capabilities}
With regard to the adversary's knowledge, we differentiate the 
\emph{white-box} from the \emph{black-box} setting: in the white-box setting, the adversary's knows everything about the training algorithm, the loss function it uses and in which way it optimizes the loss. In the black-box setting, on the other hand, the adversary does not have any intimate knowledge about the network. Instead, he has the possibility to perform a bounded number of executions on self-chosen training sets different from $D$ before he starts the attack.

The training of classifiers usually happens in an \emph{offline} fashion: the training data set $D$ is completely collected before the training and training happens only on $D$. The causative attack then tries to augment $D$ to a different data set $D'$ by either modifying, adding or removing training samples. In practice, this is a much more restrictive setting for the adversary since offline training data sets can much easier be controlled. The machine teaching framework defined by Mei and Zhu~\cite{Mei:2015:UMT:2886521.2886721} is restricted to this setting.

In \emph{online} training, we assume that there is some initial training data set $D$ that is extended by further training samples that are collected during training. In this setting, the adversary only has the option to introduce additional samples to $D$ and cannot modify or remove samples from $D$.

\boldpara{Training Data Capabilities}
We also differentiate attacks by the adversary's knowledge about the original training data set $D$. In the \emph{oblivious} case, we assume that the adversary only knows a bounded fraction of $D$, whereas in the non-oblivious case, the adversary knows the whole data set. Usually, the black-box setting excludes the possibility of having a non-oblivious attack: by having access to the full training set, the adversary can approximate the original training algorithm with another auxiliary training algorithm. 

Finally, we categorize by the options the adversary has to augment the training set $D$. He can either 
a) only modify the samples themselves,
b) change the label associated with a sample, or
c) do both.
Usually we will bound the amount of change the adversary can cause within $D$. A typical measure of change is, for instance, 
the size of the symmetric difference $\lvert D\triangle D' \rvert = \lvert D\setminus D' \cup D' \setminus D \rvert$.  



